Efficient Differentiable Programming in a Functional Array-Processing Language

We present a system for the automatic differentiation of a higher-order functional array-processing language. The core functional language underlying this system simultaneously supports both source-to-source automatic differentiation and global optimizations such as loop transformations. Thanks to this feature, we demonstrate how for some real-world machine learning and computer vision benchmarks, the system outperforms the state-of-the-art automatic differentiation tools.

==> form/ba.tex <==
\begin{figure}[t]
\hfill\begin{minipage}{.75\textwidth}\raggedright
\lett{} radialDistort = \vabs{(radical: Vector) (proj: Vector)}{}\\
\tabt \lett{} rsq = vectorNorm proj\\
\tabt \lett{} L = 1.0 + radical.[0] * rsq + radical.[1] * rsq * rsq\\
\tabt vectorSMul proj L\\
\lett{} rodriguesRotate = \vabs{(rotation: Vector) (x: Vector)}{}\\
\tabt (* Implementation omitted *)\\
% \tabt \lett{} sqtheta = vectorNorm rotation\\
% \tabt \cod{if} sqtheta != 0. \cod{then}\\
% \tabt\tabt \lett{} theta = sqrt sqtheta\\
% \tabt\tabt \lett{} thetaInv = 1.0 / theta\\
% \tabt\tabt \lett{} w = vectorSMul rotation thetaInv\\
% \tabt\tabt \lett{} wCrossX = vectorCross w x\\
% \tabt\tabt \lett{} tmp = (vectorDot w x) * (1.0 - (cos theta))\\
% \tabt\tabt \lett{} v1 = vectorSMul x (cos theta)\\
% \tabt\tabt \lett{} v2 = vectorSMul wCrossX (sin theta) \\
% \tabt\tabt vectorAdd (vectorAdd v1 v2) (vectorSMul w tmp)\\
% \tabt \cod{else} \\
% \tabt\tabt vectorAdd x (vectorCross rotation x)\\
\lett{} project = \vabs{(cam: Vector) (x: Vector)}{}\\
% \tabt\lett{} rotation = vectorSlice cam 0 2 \\
% \tabt\lett{} center = vectorSlice cam 3 5 \\
% \tabt\lett{} radical = vectorSlice cam 9 10 \\
\tabt\lett{} Xcam = rodriguesRotate (vectorSlice cam 0 2) (\\
\tabt \tabt vectorSub x (vectorSlice cam 3 5) ) \\
\tabt\lett{} distorted =  
% \\
% \tabt\tabt 
radialDistort (vectorSlice cam 9 10) ( \\
\tabt\tabt \tabt vectorSMul (%
% \\
% \tabt\tabt \tabt \tabt 
vectorSlice Xcam 0 1% 
% \\
% \tabt\tabt \tabt 
) (1.0/Xcam.[2]) ) \\
\tabt vectorAdd (vectorSlice cam 7 8) ( \\
\tabt\tabt vectorSMul distorted cam.[6]
% \\
% \tabt  
)
\end{minipage}\hfill
\caption{Bundle Adjustment functions in \lafsharp{}.}
\label{fig:ba_code}
\end{figure}

==> form/fsmooth-typesystem.tex <==
\centering
\def\comment{\hfill -- }
% \begin{flushleft}
% \textbf{Type Syntax:}
% \end{flushleft}
% \begin{subfigure}[b]{.48\textwidth}
% \begin{tabular}{r c l}
% \typet{} & ::= & \typemat{} \comment Matrix Type\\
% & | & \typefun{\typet}{\typemat} \comment Function Types (No Currying)\\
% & | & \typecard \comment Cardinality Type\\
% & | & \typebool \comment Boolean Type\\
% \end{tabular}
% \end{subfigure}
% \begin{subfigure}[b]{.50\textwidth}
% \begin{tabular}{r c l}
% \typemat{} & ::= & \typenum{} \comment Numeric Type\\
% & | & \typearray{\typemat{}} \comment Vector, Matrix, ... Type\\
% \\
% \typenum & ::= & \typedouble{} \comment Scalar Type\\
% & | & \typeindex \comment Index Type\\
% \end{tabular}
% \end{subfigure}
\centering
(T-If) $\infer{\exprind{1}: \typebool{} \tab \tab \exprind{2}: \typemat \tab \tab \exprind{3}: \typemat }{\vifthenelse{\exprind{1}}{\exprind{2}}{\exprind{3}}: \typemat}$ 
\tab
(T-Var) $\infer{\text{x}: \typet \in \Gamma }{\Gamma \vdash \text{x}: \typet}$
\\
(T-App) $\infer{\exprind{0}: \typefun{\typet}{\typemat} \tab \tab \vmore{\expr} : \vmore{\typet}}{\exprind{0}\ \vmore{\expr}: \typemat}$
\tab
(T-Abs) $\infer{ \Gamma  \cup  \vmore{\text{x}}: \vmore{\typet} \vdash \expr{}: \typemat }{\Gamma \vdash \lambda \vmore{\text{x}}. \expr: \typefun{\typet}{\typemat}}$
\\
(T-Let) $\infer{ \Gamma \vdash \exprind{1}: \typeind{1} \tab \tab \Gamma, \text{x}: \typeind{1} \vdash \exprind{2}: \typeind{2}}{\Gamma \vdash \text{\lett{} x = \exprind{1} \inn{} \exprind{2}: \typeind{2}}}$ 
% \tab \tab 
% (T-Vector) $\infer{\exprind{1}: \typemat\tab ... \tab \exprind{\valcard}: \typemat}{\varr{\exprind{1}, ..., \exprind{\valcard}}: \typearray{\typemat}}$\\

